Provable Tensor Factorization with Missing Data

We study the problem of low-rank tensor factorization in the presence of missing data. We ask the following question: how many sampled entries do we need, to efficiently and exactly reconstruct a tensor with a low-rank orthogonal decomposition? We propose a novel alternating minimization based method which iteratively refines estimates of the singular vectors. We show that under certain standard assumptions, our method can recover a three-mode $n\times n\times n$ dimensional rank-$r$ tensor exactly from $O(n^{3/2} r^5 \log^4 n)$ randomly sampled entries. In the process of proving this result, we solve two challenging sub-problems for tensors with missing data. First, in the process of analyzing the initialization step, we prove a generalization of a celebrated result by Szemer\'edie et al. on the spectrum of random graphs. Next, we prove global convergence of alternating minimization with a good initialization. Simulations suggest that the dependence of the sample size on dimensionality $n$ is indeed tight.

==> gencomplete.tex <==
\subsubsection{General Rank-$r$ Case}
\label{sec:rk}

We now present our main theorem and analysis for the general rank-$r$ case. 
Let $T=\sum_{\ell=1}^r\sol\cdot \uol \otimes \uol \otimes \uol,$  
and suppose without loss of generality that $\sigma^*_\ell\leq 1$. 
Also, let $[U,\ \Sigma]=\{(\ul, \sll), 1\leq \ell \leq r\},$ be the $t$-th step iterates of Algorithm~\ref{algo:rkk}.
%and  let $[U^{t+1},\ \Sigma^{t+1}]=\{(\ul^{t+1}, \sll^{t+1}), 1\leq \ell\leq r\}$ be the $(t+1)$-th step iterates. 
We assume that $\uo_\ell, \forall \ell$ are $\mu$-incoherent and 
$\ul, \forall \ell$ are $2\mu$-incoherent. 
Define, $\sdl=\frac{|\sll-\sol|}{\sol}$, $\ul=\uol+\dul$, $(\sdl)^{t+1}=\frac{|\sll^{t+1}-\sol|}{\sol}$, and $\ul^{t+1}=\uol+\dul^{t+1}$. 
In general, the convergence rate depends on the number of samples, 
but in any case we have linear convergence for sufficiently large sampling rate (see Figure~\ref{fig:iter}). 
Formally, the next Theorem proves this linear convergence. 
The distance is measured in 
$$d_\infty([U, \Sigma], [U^*, \Sigma^*])\;\equiv\; \max_{\ell}\left(\|\dul\|_2+\sdl\right)\;.$$ 
\begin{theorem}
\label{thm:rk}
If $d_\infty([U, \Sigma], [U^*, \Sigma^*])\leq \frac{1}{1600 r} \frac{\sigma^*_{min}}{\sigma^*_{max}}$ and $\ui$ is $2\mu$-incoherent for all $1\leq i\leq r$, then there exists a positive constant $C$ such that 
for $p\geq \frac{C r^2 (\sigma^*_{\rm max})^2 \mu^3 \log^2 n}{(\sigma_{\rm min}^*)^2 n^{3/2}}$  
%where $\gamma\leq \frac{1}{1600 r}\cdot \frac{\sigma^*_{min}}{\sigma^*_{max}}$ and $C>0$ is a global constant. 
 we have w.p. $\geq 1-\frac{1}{n^{7}}$, 
$$d_\infty([U^{t+1}, \Sigma^{t+1}], [U^*, \Sigma^*])\leq \frac{1}{2}d_\infty([U, \Sigma], [U^*, \Sigma^*]), $$
where $[U^{t+1},\ \Sigma^{t+1}]=\{(\ul^{t+1}, \sll^{t+1}), 1\leq \ell\leq r\}$ are the $(t+1)$-th step iterates of Algorithm~\ref{algo:rkk}. Moreover, each $\u^{t+1}_\ell$ is $2\mu$-incoherent for all $\ell$. 
%Let $\sdl\leq \frac{1}{200 r}\cdot \frac{\sigma_{min}^*}{\sigma_{max}^*}$ and $\|\dul\|_2\leq \frac{1}{200 r}\cdot \frac{\sigma_{min}^*}{\sigma_{max}^*}$. 
%Let $p\geq \frac{C \mu_1^3 \log^2 n}{\gamma^2 n^{1.5}}$, where $\gamma\leq \frac{1}{200 r}\cdot \frac{\sigma_{min}^*}{\sigma_{max}^*}$. Then, the following holds w.p. $\geq 1-\frac{1}{n^{7}}$: 
%$$\soq\left((\sdq)^{t+1}+\|\duq^{t+1}\|_2\right)\leq \left(\frac{1}{2}\right)^t\left((\soq\left(\|\duq^0\|_2+(\sdq)^0\right)\right)+\frac{1}{2}\left(\soll\left(\|\dull\|_2+\sdll\right)\right),$$
%where  $\ell^*=\arg\max_{\ell\neq q} \sol \left(\|\dul\|_2+\sdl\right)$. $(\sdq)^{t+1}=\frac{|\sq^{t+1}-\soq|}{\soq}$ and $(\uq)^{t+1}=\uoq+\dul^{t+1}$
\end{theorem}

\begin{figure}[h]
 \begin{center}
  \includegraphics[width=.3\textwidth]{tensor_iter}
  \put(-71,-6){iterations}
  \put(-132,50){error}
 \end{center}
 \caption{Algorithm \ref{algo:rkk} exhibits linear convergence until machine precision. 
 For the estimate $\hT_t$ at the $t$-th iterations, 
 the fit error $\|\cP_\Omega(T-\hT_t)\|_F/\|\cP_\Omega(T)\|_F$ 
 closely tracks the normalized root mean squared error $\|T-\hT_t\|_F/\|T\|_F$, 
 suggesting that it serves as a good stopping criterion.}
 \label{fig:iter}
\end{figure}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tensorcomp"
%%% End: 


==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

Define CANDECOMP/PARAFAC (CP) tensor decomposition

definition of low-rank as  CP rank


The {\em incoherence} of a symmetric tensor with orthogonal decomposition 
$T=\sum_{i=1}^r \lambda_i (u_i\otimes u_i\otimes u_i)$ is defined as 
\begin{eqnarray}
	\mu(T) &\equiv& \sqrt{\frac{n}{r}} \, \max_{i\in[n_1]} \sqrt{\sum_{j=1}^r u_{ij}^2} \;.
\label{eq:defmu}
\end{eqnarray}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tensorcomp"
%%% End: 


==> ronecomplete.tex <==
\subsubsection{Rank-one Case}

\begin{lemma}\label{lem:ip_conc}
  Let $\u, \uo\in \R^n$ be $\mu$-incoherent unit vectors. Also, let $\delta_{jk}, 1\leq j\leq n, 1\leq k\leq n$ be i.i.d. Bernoulli random variables with $\delta_{jk}=1$ w.p. $p\geq C\mu^4 \log^3n/n^2$. 

Then,  the following holds with probability $\geq 1-1/n^{10}$: 
$$|\frac{1}{p}\sum_{jk} \delta_{jk}\u_{j}\uo_{j} \u_{k} \uo_{k}-\ip{\u}{\uo}^2|\leq \gamma .$$
where $\gamma\leq C/\log n$, where $C>0$ is a global constant. 
\end{lemma}
\begin{proof}
  Let $X_{jk}=\frac{1}{p} \delta_{jk}\u_{j}\uo_{j} \u_{k} \uo_{k}.$ Note that, $|X_{jk}|\leq \frac{\mu^4}{p n^2}$. Also, $$\E[\sum_{jk}X_{jk}^2]=\frac{1}{p}\sum_{jk}(\u_{j})^2(\uo_{j})^2 (\u_{k})^2 (\uo_{k})^2\leq \frac{\mu^4}{p n^2}.$$
Hence, using Bernstein's inequality, we have: 
$$Pr(|\sum_{jk}X_{jk}-\E[\sum_{jk}X_{jk}]|>t)\leq \exp(-\frac{p n^2}{\mu^4}\cdot \frac{t^2/2}{1+t/3}).$$
Lemma now follows by selecting $t=C/\log n$. 
\end{proof}

\begin{lemma}\label{lem:ip_conc1}
  Let $\u\in \R^n$ be $\mu$-incoherent unit vectors. Also, let $a, b\in \R^n$ be s.t. $|a_i|\leq \frac{\mu}{\sqrt{n}}$ and $\|a\|_2\leq 1$.  Also, let $\delta_{jk}, 1\leq j\leq n, 1\leq k\leq n$ be i.i.d. Bernoulli random variables with $\delta_{jk}=1$ w.p. $p\geq \frac{C\mu^3}{\gamma^2 n^{1.5}}$. 

Then,  the following holds with probability $\geq 1-1/n^{10}$: 
$$|\frac{1}{p}\sum_{jk} \delta_{jk}\u_{j}a_{j} \u_{k} b_{k}-\ip{\u}{a}\ip{\u}{b}|\leq \gamma \|b\|_2.$$
where $\gamma\leq C/\log n$, where $C>0$ is a global constant. 
\end{lemma}
\begin{proof}
  Let $X_{jk}=\frac{1}{p} \delta_{jk}\u_{j}a_{j} \u_{k} b_{k}.$ Note that, $|X_{jk}|\leq \frac{\mu^3\|b\|_2}{p n^{1.5}}$. Also, $$\E[\sum_{jk}X_{jk}^2]=\frac{1}{p}\sum_{jk}(\u_{j})^2(a_{j})^2 (\u_{k})^2 (b_{k})^2\leq \frac{\mu^4\|b\|^2}{p n^2}\leq \frac{\mu^3\|b\|^2}{p n^{1.5}}.$$
Hence, using Bernstein's inequality, we have: 
$$Pr(|\sum_{jk}X_{jk}-\E[\sum_{jk}X_{jk}]|>t)\leq \exp(-\frac{p n^{1.5}}{\mu^3}\cdot \frac{t^2/2}{\|b\|_2^2+\|b\|_2t/3}).$$
Lemma now follows by selecting $t=\gamma \|b\|_2$. 
\end{proof}


\begin{theorem}
Let $p\geq C(\log^2 n)/n^{3/2}$ and let $\gamma= C/\log n\leq 1/2$. Then, after $T=\log(1/\epsilon)$ steps, alternating minimization outputs $\u^T$ s.t.: 
$\|\u^T-\uo\|\leq \epsilon$ (w.p. $\geq 1-1/n^8$). 
\end{theorem}
\begin{proof}
Let $\u^t$ be the $t$-th step update. Let $\u=\ut$. Also, let $\tu$ be obtained after $t$-th step alternating minimization step. Recall that $\u^{t+1}=\tu/\|\tu\|_2$. 

Now, using the update for alternating minimization, we have: 
  \begin{equation}
    \label{eq:r1_1}
    \tui=\frac{\sum_{(ijk)\in \Omega}\uj\uoj\uk\uok}{\sum_{(ijk)\in \Omega}(\uj)^2(\uk)^2}\uoi
  \end{equation}
Hence, 
  \begin{equation}
    \label{eq:r1_2}
    \tu=\ip{\u}{\uo}^2\uo-B^{-1}(\ip{\u}{\uo}^2B-C)\uo, 
  \end{equation}
where $B$, $C$ are diagonal matrices and $B_{ii}=\frac{1}{p}\sum_{(ijk)\in \Omega}(\uj)^2(\uk)^2$ and $C_{ii}=\frac{1}{p}\sum_{(ijk)\in \Omega}\uj\uoj\uk\uok. $

Now, using Lemma~\ref{lem:ip_conc}, we have (w.p. $\geq 1-1/n^9$): 
\begin{equation}
  \label{eq:r1_3}
  \|B^{-1}\|_2\leq (1+\gamma).  
\end{equation}

Now, 
\begin{align}
  (\ip{\u}{\uo}^2B-C)\uo=\sum_{ijk} \frac{1}{p}\delta_{ijk}\uo_i (\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uok\uj\uk) \e_i=\sum_{ijk}Z_{ijk},
\end{align}
where $Z_{ijk}= \frac{1}{p}\delta_{ijk}\uo_i (\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uok\uj\uk) \e_i$. Note that, 
$$\|Z_{ijk}\|_2\leq \frac{1}{p}\uo_i\uj\uk\sqrt{1-\ip{\u}{\uo}^4}\leq \gamma\sqrt{1-\ip{\u}{\uo}^4}, $$
where $\gamma\leq C/\log n$ and $p\geq C \mu^{3}(\log^2 n)/n^{3/2}$. 
Also, 
$$\|\sum_{ijk}\E[Z_{ijk}^TZ_{ijk}]\|_2=\| \frac{1}{p}\sum_{ijk}(\uo_i)^2(\uj)^2(\uk)^2(\ip{\u}{\uo}^2\uj\uk-\uoj\uok)^2\leq \frac{1}{p}\frac{\mu^4}{n^2}(1-\ip{\u}{\uo}^4).$$
Hence, for $p$ and $\gamma$ mentioned aboved, we have: 
$$\|\sum_{ijk}\E[Z_{ijk}^TZ_{ijk}]\|_2\leq \gamma(1-\ip{\u}{\uo}^4).$$
Using vector Bernstein inequality, we have (w.p. $\geq 1-2/n^9$): 
\begin{equation}\label{eq:r1_4}\|(\ip{\u}{\uo}^2B-C)\uo\|_2\leq \gamma\sqrt{1-\ip{\u}{\uo}^4}.\end{equation}
Using, \eqref{eq:r1_3}, \eqref{eq:r1_4}, we can bound the error term as: 
$$\|B^{-1}(\ip{\u}{\uo}^2B-C)\uo\|\leq 2\gamma \sqrt{1-\ip{\u}{\uo}^4}.$$

Hence, $(\uo)^T \tu\geq \ip{\u}{\uo}^2-2\gamma \sqrt{1-\ip{\u}{\uo}^4}$ and $(\uo_\perp)^T\tu\leq 2\gamma \sqrt{1-\ip{\u}{\uo}^4}$, where $\uo_\perp$ is any unit vector perpendicular to $\uo$. Hence, $$\sqrt{1-\ip{\u^{t+1}}{\uo}^4}\leq \frac{2\gamma}{\sqrt{(\ip{\u}{\uo}^2-2\gamma \sqrt{1-\ip{\u}{\uo}^4})^2+4\gamma^2\sqrt{1-\ip{\u}{\uo}^4}}}\cdot  \sqrt{1-\ip{\u}{\uo}^4}\leq 1/2 \sqrt{1-\ip{\u}{\uo}^4},$$
assuming $\gamma\leq 1/10$ and $\ip{\u}{\uo}^2\geq 1/2$. 

Hence, after $T=\log(1/\epsilon)$ steps, we have: $\sqrt{1-\ip{\u^T}{\uo}^4} \leq \epsilon$. 
%\begin{align}\|(\ip{\u}{\uo}^2B-C)\uo\|&=\max_{w, \|w\|_2=1} \sum_{i}w_i \uo_i (\ip{\u}{\uo}^2B_{ii}-C_{ii}),\\
%&=\max_{w, \|w\|_2=1} \frac{1}{p}\sum_{ijk}\delta_{ijk}w_i \uo_i (\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uok\uj\uk)
%\end{align}

%\begin{align}\|(\ip{\u}{\uo}^2B-C)\uo\|^2&=\sum_i  (\uo_i)^2 (\ip{\u}{\uo}^2B_{ii}-C_{ii})^2,\nonumber\\
%&= \frac{1}{p^2}\sum_{i}(\uo_i)^2 (\sum_{jk}\delta_{ijk}(\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uj\uok\uk))^2,\nonumber\\
%&= \frac{1}{p^2}\sum_{i}(\uo_i)^2 \sum_{jkj'k'}\delta_{ijk}\delta_{ij'k'}\left(\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uj\uok\uk\right)\nonumber\\&\hspace*{180pt}\left(\i%p{\u}{\uo}^2(\u_{j'})^2(\u_{k'})^2-\uo_{j'}\u_{j'}\uo_{k'}\u_{k'}\right).
%\end{align}

%Hence, 
%\begin{align}
%  \E[\|(\ip{\u}{\uo}^2B-C)\uo\|^2]&=\left(\frac{1}{p}-1\right)\sum_{jk}\left(\ip{\u}{\uo}^2(\uj)^2(\uk)^2-\uoj\uj\uok\uk\right)^2,\nonumber\\
%&\leq \left(\frac{1}{p}-1\right)\frac{\mu^4}{n^2}(1-\ip{\u}{\uo}^4).
%\end{align}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tensorcomp"
%%% End: 


==> tensorcompletioninit.tex <==
 % Tensor completion initialization 
 
We want to show that 
\begin{eqnarray*} 
	 \max_{x,y,z, \|x\|=\|y\|=\|z\|=1} \; \big( \cPO(T) - p\, T\big)[x,y,z] &\leq& C\, \Tmax\, (\log n)^2\, \sqrt{(n_1 \,n_2 \,n_3)^{1/2}\, p}\;.
 \end{eqnarray*}
 Inspired by \cite{FKS89,KMO10}, our strategy is as follows: 
 \begin{itemize}
 	\item[(1)] Reduce to $x$,$y$, and $z$ which belongs to discretized sets $\tS_{n_1}$, $\tS_{n_2}$, and $\tS_{n_3}$;
	\item[(2)] Bound the contribution of {\em light triples} using concentration of measure;
	\item[(3)] Bound the contribution of {\em heavy triples} using the discrepancy property of a random tripartite hypergraph. 
\end{itemize}

Define a discretization of an $n$-dimensional ball as
\begin{eqnarray*}
	\tS_n &\equiv& \Big\{ x\in \Big\{\frac{\Delta}{\sqrt{n}}\int \Big\}^n \;:\; \|x\|\leq 1\Big\} \;,
\end{eqnarray*}
such that $\tS_n \subseteq S_n \equiv \{x\in\reals^n\,:\, \|x\|\leq 1\}$. 
\begin{lemma}[Remark 4.1 in \cite{KMO10}]
	For any tensor $A \in\reals^{n_1\times n_2\times n_3}$, 
	\begin{eqnarray*}
		\max_{x\in S_{n_1}, y\in S_{n_2}, x\in S_{n_3}} A[x,y,z] &\leq& \max_{x\in \tS_{n_1}, y\in \tS_{n_2}, x\in \tS_{n_3}} \frac{1}{(1-\Delta)^2}A[x,y,z]
	\end{eqnarray*}
	\label{lem:disc}
\end{lemma}
It is therefore enough show that the bound holds for discretized vectors all discretized vectors $x$, $y$, and $z$.  
One caveat is that such a probabilistic bound must hold with probability sufficiently close to one such that 
we can apply the union bound 
over all discretized choices of $x$, $y$, and $z$. 
The following lemma bounds the number of such choices. 
\begin{lemma} [\cite{KMO10}] The size of the discretized set is bounded by $|T_n| \leq \big( \Delta / 10 \big)^n$. 
	\label{lem:size}
\end{lemma}
A naive approach to upper bound $(\cPO(T)-p\,T)[x,y,z]$ would be to consider it as a random variable and apply concentration inequalities directly. 
However, this naive approach fails since $x$, $y$ and $z$ can contain entries that are much larger than their typical value of $O(1/\sqrt{n})$. 
We thus separate the analysis into two contributions, and apply concentration inequalities to bound the contribution of  the {\em light triples} and 
use graph topology of the random sampling to bound the contribution of the {\em heavy triples}. 
Define the light triples as 
\begin{eqnarray}
	\cL &\equiv& \left\{ \;(i,j,k) \,:\, \big| T_{ijk} x_i y_j z_k \big| \,\leq\, \Tmax \sqrt{\frac{\eps}{n_1 \,n_2\, n_3 }} \; \right\} \;. 
	\label{eq:deflight}
\end{eqnarray}
Heavy triples are defined as its complement $\bcL = \{[n_1]\times[n_2]\times[n_3]\} \setminus \cL$. 
We can then write each contributions separately as 
\begin{eqnarray}
	\Big| \big(\cPO(T)-p\,T \big)[x,y,z] \Big| &\leq& \Big| \sum_{(i,j,k)\in\cL} \big( \cPO(T)_{ijk} x_iy_jz_k\big) - p\,T[x,y,z] \Big| + \Big| \sum_{(i,j,k)\in\bcL} \cPO(T)_{ijk} x_iy_jz_k \Big|\;. \label{eq:tcinit_separate}
\end{eqnarray}
We will prove in the following that both contributions are upper bounded by $C \Tmax (\log n)^2\sqrt{(n_1n_2n_3)^{1/2} p} $ with some positive constant $C$ 
for all $x\in \tS_{n_1}$, $y\in\tS_{n_2}$, and $z\in\tS_{n_3}$. 
Theorem \ref{thm:tcinit} then follows from Lemma \ref{lem:disc} with an appropriate choice of $\Delta = \Theta(1)$. 

See Appendix~\ref{app:init} for a detailed proof of the bounds on the light couple and heavy couple. 
%=========================================================================







%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tensorcomp"
%%% End: 

